PaperQA: Retrieval-Augmented Generative Agent for Scientific Research

Large Language Models (LLMs) generalize well across language tasks, but suffer from hallucinations and uninterpretability, making it difficult to assess their accuracy without ground-truth. Retrieval-Augmented Generation (RAG) models have been proposed to reduce hallucinations and provide provenance for how an answer was generated. Applying such models to the scientific literature may enable large-scale, systematic processing of scientific knowledge. We present PaperQA, a RAG agent for answering questions over the scientific literature. PaperQA is an agent that performs information retrieval across full-text scientific articles, assesses the relevance of sources and passages, and uses RAG to provide answers. Viewing this agent as a question answering model, we find it exceeds performance of existing LLMs and LLM agents on current science QA benchmarks. To push the field closer to how humans perform research on scientific literature, we also introduce LitQA, a more complex benchmark that requires retrieval and synthesis of information from full-text scientific papers across the literature. Finally, we demonstrate PaperQA's matches expert human researchers on LitQA.

==> sections/991-Hallucination_qs.tex <==
\section{Hallucination Testing Questions}
\begin{enumerate}
    \item Is doublecortin a unique marker of newly generated granule cells in the hippocampus?
    \item Do hair cells regenerate in wounds treated with verteporfin in mice models?
    \item In pre-commitment myeloid progenitor cells, for how many hours can estrogen be withdrawn before the cells can no longer return to their progenitor state?
    \item What effect does prenatal maternal material stress and diesel exhaust particle exposure have on the density of microglia in male mice?
    \item What effect does prenatal maternal materal stress and diesel exhaust particle exposure have on the functional heterogeneity of microglia in male mice?
    \item Between postnatal ages P6 to P15 what is the increase in thalamocortical synapse density in the anterior cingulate cortex increase in wild-type mice?
    \item What effect does infection of A. thaliana plants with avrE1/hopM1 double knockout Pst DC3000 have on NCED3 expression?
    \item What effect does infection of A. thaliana plants with avrE1−knockout Pst DC3000 have on NCED3 expression?
    \item What effect does infection of A. thaliana plants with hopM1−knockout Pst DC3000 have on NCED3 expression?
    \item Which bacterial cell wall component has been shown to facilitate lung metastasis in breast cancer models via the prostaglandin E2-EP2 pathway?
    \item When a large excess of membrane protein substrate (Vamp2) is added to the wild-type Get3/4/5 chaperone complex, the complex dissociates. Which component does the substrate not bind to?
    \item When a large excess of membrane protein substrate (Vamp2) is added to the wild-type Get3/4/5 chaperone complex, the complex dissociates into two components. Which component does the substrate bind to?
    \item In tumors with intratumoral tertiary lymphoid structures (TLS), plasma cells migrate along fibroblast conduits producing which chemokine?
    \item What fraction of chelonian species exhibit age-correlated mortality?
    \item Which of the following proteins can be used to identify Post-AIRE mTECs: Tnfaip2, Saa1, Snap25, Dynlrb2, Pdpn, or Slc12a2?
    \item I am designing peptide-guided LNPs for delivery to the retina, and am using PEG-maleimide to attach peptides to the the surface of the LNP. What fraction of the total PEG should I replace with PEG-Maleimide?
    \item How diffuse are the laminar patterns of the axonal terminations of lower Layer 5/Layer 6 intratelencephalic neurons compared to Layer 2-4 intratelencephalic neurons in mouse cortex?
    \item Following consumption of a meal shake, how long after consumption do the majority of significantly altered lipids reach their peak levels?
    \item Roughly what fraction of Jun molecules degrade over 4 hours in HEK293T cells?
    \item What kind of protease do SNIPRs depend on for activation?
    \item What fraction of dopaminergic neurons in the mushroom body receive input from all sensory modalities?
    \item What fraction of octopaminergic neurons in the mushroom body receive input from all sensory modalities?
    \item What fraction of transcription factor isoforms can significantly alter pseudotime upon overexpression in hESC differentiation?
    \item Which of the following drugs can NOT be used to inhibit binding of the viral protease dNS3S139A to the antiviral peptide CP5-46A-4D5E: Grazoprevir, Glecaprevir, Danoprevir, or Telaprevir?
    \item Which of these glycoRNAs does NOT show an increase in M0 macrophages upon stimulation with LPS: U1, U35a, Y5 or U8?
    \item In the ARPLA method for detecting surface glycoRNAs, what glycan does the aptamer bind?
    \item How many clades of adenosine deaminases are there when grouped according to structure-based clustering?
    \item Which of the following compounds is most effective at enhancing ER proteostasis and promote functional, soluble forms of GCase in neurons - DANT, DHBP or DILT?
    \item What is the substrate preference of the Ddd1 deaminase?
    \item Which reactive astrocyte marker has been shown to increase in expression in RhoAnesKO mice?
    \item Neonatal male mice injected with NIF, a glycoprotein produced by a canine hookworm, show a significant reduction in microglial phagocytic capacity and engulfment of which neurotransmitter transporter?
    \item In 5XFAD mice, what effect does microglia-specific Ifnar1 deletion have on post-synatptic terminals?
    \item In 5XFAD mice, what effect does neural Ifnar1 deletion have on pre-synatptic terminals?
    \item Which over-the-counter antihistamine has been found to be as effective as anti-VISTA antibodies in prolonging survival of mice and inhibiting lung metastasis when combined with ICB therapy?
    \item Which of the following genes shows the greatest difference in gene expression between homologous cell types in mouse and human brain: Htr3a, Htr1d, Htr5a, or Htr6?
    \item What fraction of bipolar interneuron axons target other interneurons in the human temporal and frontal cortex?
    \item Which of the following genes has been shown to be localized to granule cells in the cerebellum that are anterior to the primary fissure: Aldoc, Rasgrf1, Plcb4, or Mybpc1?
    \item Which of the following genes has been shown to be a specific marker for parvalbumin interneurons in the molecular and fusiform layers of the dorsal cochlear nucleus: atp9a, Atp5b1, Atp6v1g2, or Atp2b1?
    \item Has anyone performed a base editing screen against splice sites in CD33 before?
    \item Is it possible to do tagmentation of cDNA directly in the PCR mix without cleaning and quantifying the cDNA first?
    \item In the Ingraham 2022 protein design paper, how did they force the protein complexes to be symmetric with respect to a specific space group?
    \item What percentage of colorectal cancer-associated fibroblasts typically survive at 2 weeks if cultured with the platinum-based chemeotherapy oxaliplatin?
    \item Which three residues with evolutionary divergence in the G domains of RAS isoforms also impose selectivity constraints of pan-KRAS non-covalent inhibition?
    \item What are possible targets of the immunostimulatory molecule in immune-stimulating antibody conjugates?
    \item How is Bempegaldesleukin supposed to overcome Treg affinity for IL-2?
    \item How many FMD cycles are the minimum required to cause a significant delay in the growth of melanoma tumors in mice?
    \item Based on the single-cell transcriptome analysis highlighting fatty acid metabolism-mediated metastasis and immunosuppression in male breast cancer, what percentage of ER+ MBC patients showed AR-negative status when evaluated by IHR?
    \item Does metabolic glycan labeling immobilize dendritic cell membrane and enhance antitumor efficacy of dendritic cell vaccine?
    \item Which mouse model(s) of immunisation was used to demonstrate CD90 could identify germinal center-resident follicular helper CD4+ T cells?
    \item What is the net rate of 3D imaging for time-lapse continuous data generated by 2pSAM (Two-photon Synthetic Aperture Microscopy)?
    \item What marker combination that includes CD38 can be used to identify murine liver CD8+ tissue-resident memory T cells independent of CD69 during inflammatory conditions?
    \item If implementing symmetric molecular dynamics as a holonomic constraint, how can Wyckoff sites be constrained?
\end{enumerate}

==> tables/medqa-results.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
    \begin{tabular}{l lcc}
        \toprule
         Method & Details & MedQA-USMLE & BioASQ \\
         \midrule
         Galactica & Finetuned & 44.4 & 94.3 \\
         BioLinkBERT & Finetuned & 44.6 & 94.8\\
         Codex & 5-shot & 46.1 & -- \\
         GPT-3.5 & 0-shot & 50.8 & 85.0\\
         GPT-3.5 & 5-shot & 53.6 & --\\
         GPT-4 & 0-shot & 84.4 & 91.0 \\
         GPT-4 & 5-shot & 86.1 & --\\
         Med-PaLM 2 & & 86.5 & --\\
         \midrule
         \textbf{PaperQA} & Sample of 40 & 62.0 & 76.0\\
         \textbf{PaperQA} & Upper bound (parsing fix..) & 76.0 & 92.0\\
         \midrule
         Human (passing) & & 60.0 & --\\
         Human (expert) & & 87.0 & --\\
        \bottomrule
    \end{tabular}
    \label{tab:visor_main}
\end{table*}
